The Effects of Hallucinations in Synthetic Training Data for Relation Extraction

Relation extraction is crucial for constructing knowledge graphs, with large high-quality datasets serving as the foundation for training, fine-tuning, and evaluating models. Generative data augmentation (GDA) is a common approach to expand such datasets. However, this approach often introduces hallucinations, such as spurious facts, whose impact on relation extraction remains underexplored. In this paper, we examine the effects of hallucinations on the performance of relation extraction on the document and sentence levels. Our empirical study reveals that hallucinations considerably compromise the ability of models to extract relations from text, with recall reductions between 19.1% and 39.2%. We identify that relevant hallucinations impair the model's performance, while irrelevant hallucinations have a minimal impact. Additionally, we develop methods for the detection of hallucinations to improve data quality and model performance. Our approaches successfully classify texts as either 'hallucinated' or 'clean,' achieving high F1-scores of 83.8% and 92.2%. These methods not only assist in removing hallucinations but also help in estimating their prevalence within datasets, which is crucial for selecting high-quality data. Overall, our work confirms the profound impact of relevant hallucinations on the effectiveness of relation extraction models.

==> 4_Approach.tex <==
\section{Approach}
\label{sec:approach}

To assess the impact of hallucinations on synthetic training data for relation extraction, it is crucial to determine their qualitative effect on the language models trained with such data (referenced as RQ1). We address this by comparing model performance using datasets characterized by varying levels of hallucinations.

Our second research question (RQ2) focuses on developing a method to measure the prevalence of hallucinations within the data. We explore various metrics designed to detect and quantify these hallucinations. This quantification enables us to eliminate data points contaminated by hallucinations and to forecast the performance of relation extraction models based on the hallucination density in their training datasets. In the following, we first present our approach for RQ1, followed by our approach for RQ2.




\subsection{Measuring an Effect of Hallucinations}
\label{App: Measuring an Effect of Hallucinations in the Training of Relation Extraction models}



The concept of hallucinations lacks a universally accepted definition \cite{ji_survey_2023, filippova_controlled_2020, nie_simple_2019, ye_cognitive_2023, shuster_retrieval_2021}. 
Figure \ref{fig:example_hallucination} provides an example of a hallucination. In this scenario, a GDA model, tasked with generating text from the input triple ('Ted', 'lives in', 'New York'), should ideally produce 'Ted lives in the city of New York.' Instead, the model might extend this to 'Ted lives in the city of New York, which has a population of 8.4 million inhabitants.' This addition introduces an unsupported triple ('New York', 'has', '8.4 million inhabitants'), which is a hallucination.

Formally, we define hallucinations $H$ as the set difference $ H = TC \setminus T$ between the set of triples $T$ and the triples $TC$ that are actually generated in the text $S$. Hallucinations are identified only when $TC$ exceeds $T$ in content, not the other way around.







We differentiate between relevant and irrelevant hallucinations in relation extraction models, illustrated in Figure \ref{fig:relevant_irrelevant_hallucinations}. These models are typically optimized to identify specific types of relations, which we define as relevant relations \cite{clive_control_2022,yan_partition_2021}. Relations that do not pertain to the model's intended use are classified as irrelevant.

Relevant hallucinations occur when texts express triples with relevant relation types that are absent in the annotations. For example, if a model is trained exclusively to detect dates of birth in texts, only triples related to this information are considered relevant. Conversely, irrelevant hallucinations involve relations that the model is designed to ignore, as these do not pertain to its trained focus.

In our work, we consider datasets that include both relevant and irrelevant types of hallucinations to better understand how relation extraction models selectively process information. 

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.75\linewidth]{images/Figures/Relevant_irrelevant_hallucinations.drawio.png}
    \caption[Illustration of the distinction between relevant and irrelevant hallucinations in a dataset]{This figure illustrates the distinction between relevant and irrelevant hallucinations in a dataset. It presents two examples of hallucinations, one with an irrelevant relation type, 'occupation,' and the other with a relevant relation type, 'birthDate.'}
    \label{fig:relevant_irrelevant_hallucinations}
\end{figure}


\textbf{Approach.} To investigate the effects of hallucinations on relation extraction models, we design an experiment using datasets that exhibit varying degrees of hallucinations. We aim to train relation extraction models on these datasets to discern the impact of hallucinations on model performance, maintaining minimal variables in our experiment setup to ensure that any performance differences can be attributed solely to the presence of hallucinations.

Initially, we identify and prepare suitable datasets for relation extraction, ensuring that they conform to our criteria regarding the presence of hallucinations. Both datasets are then used to fine-tune Pretrained Language Models (PLMs) using a consistent training protocol, resulting in two model configurations adapted to distinct datasets.

Subsequently, we compare these configurations using widely recognized metrics in relation extraction—precision, recall, and F1-Score \cite{josifoski_exploiting_2023, brown_language_2020, xu_how_2023, park_improving_2021}. As more hallucinations are present, we expect the models to demonstrate variations in their ability to discern relevant information, potentially leading to a decrease in recall due to the model's learned tendency to overlook non-annotated data, thereby affecting the number of true positives detected.







\subsubsection{General Structure of the Datasets}
\label{App: General Structure of the Datasets}

Figure \ref{fig:datasetstructure_training} shows the structure of our datasets. We require datasets with a low incidence of hallucinations to ensure that the annotated triples accurately describe the corresponding textual content. We will call these datasets $A$ and refer to them as 'clean datasets.' For each clean dataset, we then need a nearly identical dataset $B$, where the only difference from $A$ is an increase in the amount of hallucinations. This results in incomplete annotations that do not cover all the information from the text fields of $B$.  

Further, we use different datasets to test the distinct types of hallucinations. These datasets contain either relevant or irrelevant hallucinations, allowing for a precise evaluation and subsumption of the effects of each hallucination type. 

In this paper, we divide each dataset into two parts: training and test sets. The training set contains the majority of the data and is the most relevant for our purposes, as it is the part that is mostly modified and used for training. The test set is used to evaluate the resulting fine-tuned language models and remains mostly unchanged. When referring to any dataset, such as A or B, we always refer to the training component of the dataset. When referring to the test component of the dataset, we will use the notation $DatasetName^{test}$. Also, when B consists of more than one dataset, we will refer to it as $B_{fused}$.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.75\linewidth]{images/Figures/Approach_Datasetstructure_Training.drawio.png}
    \caption[Illustration of the approach used for testing the influence of hallucinations]{This figure illustrates the approach used for testing the influence of hallucinations with the datasets A and B and the language models trained on them.}
    \label{fig:datasetstructure_training}
\end{figure}





\subsubsection{Testing the Effects of Relevant Hallucinations}
\label{App: Testing the Effects of Relevant Hallucinations}

In this section, we conduct experiments to see if the impact of relevant hallucinations on relation extraction model performance can be measured.


\paragraph{Dataset Structure}

We use two datasets, A and B, for each test. They should be designed or viable for relation extraction. Additionally, we alter A and B to test if effects can be measured for various datasets and to exclude the chance of unwanted dataset-specific influences on the training performance of the relation extraction models.

\paragraph{Training Procedure}

For the training, a suitable relation extraction approach M has to be found to fine-tune it on the clean dataset A. Then, the same approach, M, is fine-tuned on dataset B, which contains more hallucinations, using the same training procedure.\\
Finally, the performance of M$_{A}$ and M$_{B}$ must be compared on the clean A$^{test}$ dataset to determine if the hallucinations in the texts affect the training results.
This is repeated after the alteration of A and B.

\paragraph{Differences Between Variants of A and B}

\textbf{Setting 1:} For the first experiment, datasets A and B should not need to be modified. For this purpose, an old and a new version of the same dataset can be used. In that case, B must have some missing triples in the annotation. At the same time, A should be an improved version of dataset B with a more complete annotation and, therefore, have fewer relevant hallucinations.

With this preparation, we can run early experiments with minimal time and effort and see if there are any differences in performance between models trained on A and B. If not, it is very likely that hallucinations do not affect the performance of the models trained on them. Conversely, further investigation using the following datasets is important and necessary if there are differences. 

\textbf{Setting 2:} For the next experiment, we need to alter A and B. A will serve as the basis for all subsequent datasets to optimally control for specific conditions when creating modifications.
Therefore, A should be a dataset suitable for relation extraction tasks with minimal hallucinations, ideally with no relevant hallucinations at all.
With A as a basis, we create two variants for B: B$_{MT}$ and B$_{LT}$, which will be together referred to as $B_{fused}$. The first has missing triples, and the other has longer texts. \par
The B$_{MT}$ dataset is created to evaluate relevant hallucinations accurately. To achieve this, triples are removed from the annotations. We chose this procedure since it accomplishes two things. Firstly, it creates relevant hallucinations due to missing crucial information in the annotations. Secondly, it helps quantify the amount of hallucinations since we know how many triples have been removed.\par

Due to the creation process of B$_{MT}$, there may be an alternative explanation for a performance drop besides the increase in hallucinations. The difference between A and B$_{MT}$ lies in the number of triples included in the annotations of the texts. Therefore, an relation extraction approach trained on A will have significantly more examples of triples than when trained on B$_{MT}$, which might contribute to a difference in performance. To investigate this possibility, we create B$_{LT}$.\par

To test for the possibility explained above, it is important that the set of triples T from A remains unchanged. Hence, B$_{LT}$ requires different means than B$_{MT}$ for the creation of relevant hallucinations. One possible and easily implemented solution that satisfies our needs is to expand S by incorporating additional texts S2 from other data points of A. This results in an increase in the length of S as well as the number of relevant triples it contains, while still preserving T.


\subsubsection{Testing the Effects of Irrelevant Hallucinations}
\label{App: Testing the Effects of Irrelevant Hallucinations}

For the second hallucination type, we produce hallucinations in a similar manner as GDA could.

\subparagraph{Dataset Structure}

We do not need to adjust A for this part, but the B dataset must undergo significant alterations. 
Five datasets with irrelevant hallucinations are created, which together represent B. To ensure comparability with the goal of evaluating unintentional hallucinations by GDA, a large language model is used to create them. To achieve this, each data point from A, consisting of S and T, is used as an input prompt for the LLM. The LLM adds information to S that is not present in T, leading to hallucinations. We iteratively modify the prompt to obtain better and more diverse results, creating multiple datasets. Our approach is designed to produce primarily irrelevant hallucinations. However, it is not possible to know the exact composition of the resulting hallucinations since the LLM cannot be controlled to such an extent.

In addition to A$^{test}$, a second and new test dataset must be created. This ensures that any differences in results between relation extraction approach M trained on A and M trained on B are only influenced by the different amounts of hallucinations in the datasets. The LLM mainly adds irrelevant hallucinations at the end of texts, so it is possible that during the training process, M$_{B}$ learns to ignore the last part of long texts and extracts only triples from the first part. Therefore, the model does not learn to ignore irrelevant hallucinations but only a specific position in the texts.
A new test dataset is created to test for this bias by merging different data points from A$^{test}$. This results in a test set where all data points have longer texts and more extended annotations without introducing new hallucinations compared to A$^{test}$.
If M$_{B}$ were to learn to ignore certain parts of the text, it would perform worse on the new test dataset than M$_{A}$, as it would extract fewer triples.

\subparagraph{Training Procedure}

The training process can be replicated similarly to the previous experiments. 
Also, the same relation extraction approach, M, can be utilized since the base dataset remains unchanged.


\subsection{Creating Metrics for Hallucination Detection and Quantification}
\label{App: Creating Metrics for Hallucination Detection and Quantification}

This section aims to evaluate and test if hallucinations in \gls{td} can be detected and their amount quantified using specific metrics. 
Such a metric would allow for the removal of corrupted data from a dataset and, therefore, improve its quality.
Additionally, the metric would allow a comparison between the performance of language models and the amount of hallucinations in the datasets they were trained on in Section \ref{App: Measuring an Effect of Hallucinations in the Training of Relation Extraction models}. That way, the impact of hallucinations can be further quantified, and their effect on other relation extraction approaches can be anticipated.


\subsubsection{Difference between Hallucination Detection and Quantification}
\label{App: Difference between Hallucination Detection and Quantification}

We split the overall task of detection and quantification of hallucinations into two separate tasks. To understand why, we must consider our main objective and the difficulties in quantifying hallucinations. Generally, we aim to identify triples in S that are not in TC and could potentially affect the training performance of relation extraction models. It is currently unclear whether relevant or irrelevant hallucinations have an impact and to what extent. Hence, it might be crucial only to identify relevant hallucinations while ignoring irrelevant ones. \par

However, identifying general hallucinations seems logically much easier than identifying only relevant ones since there is no need to distinguish between relevant and irrelevant relations. For the detection of hallucinations, it is enough if TC has more triples than T. That way, we know if there are hallucinations in the text, but not to what extent.
However, when quantifying hallucinations, we need to determine the number of triples missing in the annotation. Furthermore, it may be necessary to distinguish between missing relevant or irrelevant information since only the relevant information might be meaningful for the impact on performance. Since detecting hallucinations is necessary to quantify them, quantifying them can logically not be easier than detecting them.\par
If there were a perfect relation extraction model, extracting every triple and comparing it to those in T would be easy, thereby solving both tasks concurrently. However, since none of the widely used relation extraction datasets like Re-DocRED \cite{tan_revisiting_2022, redocred_papers_2024}, TacRED \cite{zhang_position-aware_2017, tacred_papers_nodate} or Re-TacRED \cite{stoica_re-tacred_2021, re-tacred_papers_nodate} show perfect relation extraction models, this is not possible and alternative methods must be explored. \par

To achieve our goal and answer whether it is possible to quantify hallucinations, we begin with the more fundamental task of detecting them. This allows us to determine if a solution is feasible and identify reliable components for the more challenging task.


\subsubsection{Detection of Hallucinations}
\label{App: Detection of Hallucinations}

To detect hallucinations, we first need to create a suitable dataset to test the metrics.

\paragraph{Structure of the Dataset}
\label{App: Structure of the Dataset (detection)}
The dataset D must meet the following criteria:
\begin{enumerate}
    \item The general structure has to contain triple and text pairs as data points.
    \item It needs to have clean text for each set of triples. This implies that it can neither contain irrelevant nor relevant hallucinations.
    \item There has to exist a text with hallucinations in addition to the clean text for each list of triples.
\end{enumerate}
With the first point, we ensure that the dataset remains consistent with the actual relation extraction datasets, which always include those two elements in each data point \cite{stoica_re-tacred_2021, tan_revisiting_2022, gardent_webnlg_2017}.
The next two requirements allow for the testing of the metrics in the following ways. First, the ability to accurately classify a hallucination as 'hallucination.' Second, the ability to correctly identify texts without hallucinations as 'clean.'\par
To meet the three requirements, we create dataset D with the structure depicted in Figure \ref{fig:dataset_metric_detection}. The data consists of data points, each containing a tuple (T, L) with a list of triples as T and a set of two elements: 'clean' and 'hallucination,' as L.
The 'clean' elements must only consist of clean texts (one or more). The 'hallucination' elements must contain text with a small or considerable amount of hallucinations.\\
To create a dataset D in this format, an existing relation extraction or knowledge graph-to-text dataset D0, which is free of hallucinations, can be used. The requirement for D0 is that it must contain lists of triples T1 that are part of other lists of triples T2, which means it must fulfill $T1 \subset T2$ for some elements. Then modify D0 as follows:\\
Each list of triples T1 and their corresponding clean texts c can be added to the new dataset D. For the 'hallucination' elements h of each data point, we must find texts that contain the same triples as T1 and some additional Information. For that, another data point that contains T2 has to be found in D0. Then, the corresponding text can be added to h.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.9\linewidth]{images/Figures/Datensatz_Metrik.drawio.png}
    \caption[Illustration of the structure of the dataset D for hallucination detection]{This figure illustrates the structure of the dataset D for hallucination detection. Each data point of the dataset consists of a set of triples T and a set of two texts L. L contains a clean text without hallucinations c and a text with hallucinations h}
    \label{fig:dataset_metric_detection}
\end{figure}

\paragraph{Possible Solutions for Detecting Hallucinations}
\label{App: Possible Solutions for Detecting Hallucinations}

All methods presented are evaluated for their suitability or potential for adjustment, and the most effective is determined. Two approaches are utilized to detect hallucinations. 

\subparagraph{NER Approach}

A less precise but more dependable solution to relation extraction is to use a named entity recognition model (NER model), as suggested by Liu et al. \cite{liu_towards_2021} and introduced in Section \ref{RW: Hallucinations}. This model allows for the extraction of all entities from a given text, which can then be compared to the entities contained in the triples belonging to the text. If any entities are extracted from the text but not included in the triples, they are considered hallucinations. It is important to note that the extracted entities may not be in the same form as those in the triples. Therefore, a tool for detecting sentence similarity or equivalences in meaning must be used to compare the extracted and already present entities. \par

\subparagraph{Textual Entailment Approach}

Another approach inspired by Dušek and Kasner \cite{dusek_evaluating_2020} is to utilize an entailment model M, that determines if a given sentence is part of another sentence. For the functionality of Entailment Models, refer to Section \ref{Foun: Textual Entailment}. In our case, we can use it to verify if S contains the same information as T. To accomplish this, we combine all triples $t \in T$ into a single sentence by linking them with a conjunction so that each triple is connected with the next triple. If M classifies T as not entailed, that means it has hallucinations. Conversely, if T is classified as entailed, then S must be hallucinations-free.\par

This method allows us to determine the number of data points in a dataset that contain hallucinations, providing an approximate idea of the total amount of hallucinations in the dataset. However, it cannot measure the amount of hallucinations in specific data points.\par




\subsubsection{Quantification of Hallucinations}
\label{App: Quantification of Hallucinations}

To quantify hallucinations, we present the \textbf{E}ntailment and \textbf{N}amed \textbf{E}ntity \textbf{R}ecognition (ENER) approach, which combines the textual entailment approach with the NER approach.\par

Since the dataset from the previous section lacks a specification for the amount of hallucinations in h, we require an additional dataset to evaluate the metric in quantifying the number of relevant hallucinations.

\begin{figure}
    \numberwithin{figure}{section}
    \centering
    \includegraphics[width=0.8\linewidth]{images/Figures/Datensatz2_Metrik.drawio.png}
    \caption[Illustration of the structure of the dataset D for hallucination quantification.]{This figure illustrates the structure of the dataset D for hallucination quantification. Each data point of the dataset consists of a set of triples T, a natural language text with hallucinations S, and a set of missing triples MT, that contains all the hallucinations of S}
    \label{fig:dataset_metric_quantification}
\end{figure}

\paragraph{Structure of the Dataset}
\label{App: Structure of the Dataset (quantification)}

The new dataset D must meet the following criteria:
\begin{enumerate}
    \item The general structure has to contain triple (annotation) and text pairs as data points.
    \item All triples contained in the texts have to be known.
    \item A significant amount of annotations has to have missing triples
    \item Each data point must contain all triples that are missing in the annotation
\end{enumerate}
The first requirement has the same reasoning as in the previous dataset in Section \ref{App: Structure of the Dataset (detection)}. However, the following three requirements ensure that the dataset containing hallucinations can be used for testing. By including all text-contained triples in the data points, we can reliably check if our new metric can find them and determine how closely the metrics results match reality. 
To achieve D (see Figure \ref{fig:dataset_metric_quantification}), we use a dataset without any hallucinations as a basis. We then randomly delete triples from the annotations and save the deleted triples in MT, which is part of the same data point. This allows us to obtain relevant hallucinations while knowing the exact extent of missing relevant triples.


\paragraph{ENER Approach}
\label{App: Possible Solution for The Quantification of Hallucinations}

To illustrate the following concept, an example is presented in Figure \ref{fig:approach_ENER}.
This metric is designed to quantify the number of relevant hallucinations in a text and distinguish between relevant and irrelevant hallucinations. It takes as input a dataset consisting of T and S, as well as a list of all relevant relations R. It can determine the absolute and relative amount of triples missing in the annotations of the dataset. The approach consists of three steps. First, all entities contained in S are extracted to get the set E. In step two, to form triples, every $e_{1} \in E$ is combined as head entity with every $e_{2} \in E$, $e_{1} \neq e_{2}$ as tail entity through every $r \in R$ as relation. This procedure creates ST, a set of all possible relevant triples. In the last step, the entailment model checks for each $t \in ST$ whether t is contained in S. If not, the triple is discarded, and the next one is in line. If it is contained in S, a relevant missing triple t$_{r}$ is found and thus a relevant hallucination. This process is repeated for each data point.\par


\begin{figure}
    \numberwithin{figure}{section}
    \centering
    \includegraphics[width=0.8\linewidth]{images/Figures/Approach_ENER.drawio.png}
    \caption[Illustration of the ENER approach with an example]{This figure illustrates the ENER approach with an example. 
    First, all entities are extracted to test the number of relevant hallucinations in the given text. Afterward, all possible triples are constructed using 'birthDate' as a relation and the extracted entities as head and tail entities. In the last step, for each triple $t \notin T \land t \in ST$, the entailment model checks whether t is contained in S. That way, the relevant hallucination ('Nikola Tesla', 'birthDate', 'Juli 10, 1856') is found.}
    \label{fig:approach_ENER}
\end{figure}

\subsection{Summary}

In this section, we introduced our approaches for:

\begin{enumerate}
    \item A distinction between different kinds of hallucinations, namely relevant and irrelevant hallucinations.
    \item Testing whether an effect of hallucinations on various relation extraction tasks can be measured.
    \item To find differences in the influence of relevant and irrelevant hallucinations.
    \item The creation of multiple relation extraction datasets with varying amounts of relevant and irrelevant hallucinations to test their effects.
    \item Detecting and quantifying hallucinations in a dataset.
    \item The creation of datasets to test the metrics for detecting and quantifying hallucinations.
\end{enumerate}


==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> images/txts/ENER_results.tex <==
Threshold	Recall	Precision	F1
0.05	2.63	94.12	5.11
0.1	2.93	97.41	5.69
0.15	3.15	94.95	6.10
0.2	2.54	94.89	4.93
0.25	2.35	96.21	4.59
0.3	2.96	94.30	5.74
0.35	3.03	95.40	5.88
0.4	3.02	94.38	5.86
0.45	2.73	92.73	5.29
0.5	3.64	92.77	7.01
0.55	4.82	95.86	9.18
0.6	5.10	93.00	9.67
0.65	7.34	91.07	13.59
0.7	7.09	90.79	13.15
0.75	13.64	90.05	23.68
0.8	14.16	84.16	24.22
0.85	19.40	78.91	31.12
0.9	31.70	72.56	44.06
0.91	39.19	73.73	49.89
0.92	36.85	68.73	47.14
0.93	44.04	64.95	52.47
0.94	44.21	62.82	51.84
0.95	55.03	60.43	57.41
0.96	58.07	53.38	55.62
0.97	58.72	41.12	48.35
0.98	66.55	40.31	50.11
0.99	80.65	18.02	29.45

